Controlling Tail Risk in Online Ski-Rental

The classical ski-rental problem admits a textbook 2-competitive deterministic algorithm, and a simple randomized algorithm that is $\frac{e}{e-1}$-competitive in expectation. The randomized algorithm, while optimal in expectation, has a large variance in its performance: it has more than a 37% chance of competitive ratio exceeding 2, and a $\Theta(1/n)$ chance of the competitive ratio exceeding $n$! We ask what happens to the optimal solution if we insist that the tail risk, i.e., the chance of the competitive ratio exceeding a specific value, is bounded by some constant $\delta$. We find that this additional modification significantly changes the structure of the optimal solution. The probability of purchasing skis on a given day becomes non-monotone, discontinuous, and arbitrarily large (for sufficiently small tail risk $\delta$ and large purchase cost $n$).

==> intro-old.tex <==
\section{Introduction}
\label{sec:intro}
Consider the classical ski-rental problem -- every morning Alice must decide whether to rent skis for \$1 or buy them for \$n, in which case she never needs to rent them again. Her choice is non-obvious because she does not know how many days she is going to ski --- the weather may be too warm, she may get injured, or may just tire of the sport. Folklore analysis says that committing to buy skis on the morning of day $n$ is (deterministically) optimal, as Alice never over-spends by more than a factor of 2, no matter how many days she ends up skiing. 

If Alice is willing to randomize, then she can commit to buy the skis  on day $i\in [n]$ with probability proportional to $\exp(i/n)$. This method gives a $\nicefrac{e}{e-1} \approx 1.58$ competitive ratio. On its face, this is significantly better, however, following the randomized strategy Alice incurs significant {\em tail risk}. In fact, while on average, the competitive ratio is $1.58$, there is a more than $37\%$ probability that her competitive ratio will be above 2 (i.e. worse than the deterministic algorithm), and more than a 16\% probability that the competitive ratio will be above 4. in fact, her worst case ratio is unbounded -- for any $\gamma > 2$ there's a $\frac{e^{\nicefrac{1}{\gamma}} - 1}{e - 1} \geq \frac{1}{\gamma (e-1)}$ probability of the competitive ratio exceeding it.  

As such the randomized algorithm, while optimal in an expected sense, is hard to recommend to a practitioner\thomas{I like this, but maybe need more context to connect to practice'}. To control for these low probability bad outcomes a natural approach is to put an explicit constraint on the tail of the competitive ratio random variable. Let a $(\gamma, \delta)$-tail constraint denote the restriction that the probability (over the choices made by the algorithm) that the worst-case competitive ratio exceeds $\gamma$ is at most $\delta$. The question that we ask in this work is how do such restrictions change both the competitive ratio, and the optimal algorithm itself. Even for the simple question of ski-rental, the optimal solution is non-obvious: as we will show the for non-trivial $\delta$ and $\gamma$ the optimal distribution is non-monotone, and non-convex. In fact, it will have days with {\em zero} probability of buying skis, and others with ever growing probability of purchase. 

\mdnoteinline{
I agree with Sergei that the above isn't punchy enough.  I don't have time right now to do a full rewrite, but here's the story that I was thinking of. 

\ \\


Online algorithms are an influential and important topic of study in TCS.  Starting from (citation), they have played a huge role in the development of the theory of algorithms.  While the paging problem is perhaps the most foundational ``applied'' online problem, the simplest, most basic online problem is the \emph{Ski Rental} problem.  In this problem, etc.\ etc.  There is a deterministic $2$-competitive algorithm, and a randomized $e/(e-1)$-competitive algorithm.

Ski rental was not only the first online problem to be studied in the context of competitive analysis, it is also usually the first online setting taught to students.  This is because it is essentially the simplest possible setting where ``not knowing the future'' can lead to a huge cost in performance, but where clever algorithms can mitigate this and still allow for high-quality worst-case bounds.  Moreover, it is one of the simplest settings in which it is possible to show that randomness gives us more power.

Based on its age and status as the simplest problem in online algorithms, one might expect that essentially everything is known about ski rental.  Indeed, modern research on ski rental has generalized it to a number of interesting settings (citations), but to the best of our knowledge there have not been any new results on the basic ski rental problem itself in a number of years.  

In this paper we revisit the classical ski rental problem for the first time in x years, studying the basic problem but under more refined probabilistic analysis: we study the \emph{tail} of the randomized algorithm rather than just its expectation.  Tail bounds are of central importance in the study of online algorithms, but to the best of our knowledge there has been no study of tail bounds of ski rental.  This is despite the fact that they are even better motivated in the online setting than in the traditional computational model, since in the online setting we cannot simple repeat the algorithm more times in order to gain concentration.  Indeed, it turns out to be siple to argue that the traditional randomized algorithm, with expected competitive ratio of $e/(e-1)$, has an almost 37\% chance of have competitive ratio larger than $2$, i.e., of actually being \emph{worse} than the simple, deterministic $2$-competitive algorithm!

Sergei's paragraph about practitioner / tail risk.

In this paper we initiate the study of tail bounds for ski rental.  We provide optimal algorithms for any combination of tail risk constraints, but more interestingly we show that adding tail bounds actually \emph{changes the structure} of the optimal solution is surprising and interesting ways.  One obvious method to obtain tail bounds is simply to use a linear interpolation of the classical randomized and classical determoinistic algorithms.  This would have a number of properties which one might expect any ``reasonable'' randomized algorithm to have: the probability mass is monotonically increasing in time, is never $0$ at any point in time, and grows at a ``reasonable'' rate.  In contrast, we show that the optimal algorithm in the presence of even a single tail bound has \emph{none} of these properties!  It is not monotonically nondecreasing, it can drop to $0$ an arbitrarily large number of times, and it can grow arbitrarily fast.
}

\subsection{Our Results}
Recall the randomized algorithm for ski-rental. Prior to the first day of skiing, Alice flips a coin and commits to buying skis on the morning of day $i$ with probability $f_i$. We call $f = \{f_i\}_{i\in [n]}$, the purchase distribution. For the purpose of the analysis, for a given $f$ it will be helpful to consider the competitiveness function, $\alpha_f$, where $\alpha_f(x)$ is the expected competitive ratio when Alice stops skiing at the end of day $x$. 

The randomized algorithm minimizing the expected competitive ratio, i.e. $\max_x \alpha_f(x)$ sets $f_i \propto \exp(i/n)$\sergei{not sure about off the discrete case}. The optimal choice of $f$ balances two competing objectives -- buying early is good if the number of skiing days exceeds $n$, on the other hand, buying late is good if the adversary's choice is small. The balance is done in the worst-case over all adversary's choices, but in expectation over the random coins flipped by the algorithm. In the optimal solution the balance has the effect that the competitiveness function, $\alpha$ is constant over the time period from $1$ to $n$. 

Now suppose we wish to enforce a $(\gamma, \delta)$-tail constraint. For a given purchase distribution $f$, with probability $f_i$ the algorithm buys early on day $i$. However, in this case $\alpha_f(i)$, i.e. the competitive ratio when the adversary chooses $i$ as the last skiing day is $(n + (i-1))/i$. If this value exceeds $\gamma$ then this event must be accounted as part of the tail-risk. What we will show is that the competitiveness function $\alpha$ is no longer constant in an optimal solution. 

\paragraph{General Tail Constraints} 
We begin by characterizing the optimal solution. Our proof proceeds by a careful analysis of the competitiveness function, $\alpha$. We first show that $\alpha_f(x)$ depends only the values of $f_i$ for $i \leq x$. This follows intuition---from the point of view of season ending at $x$ the only thing that matters is the probability that Alice kept renting at $x$. The exact time $t > x$ that she committed to buy the skis is not important. 

We then show that no matter the number and shape of tail constraints, for an optimal solution, $f^*$, with value $OPT$, $\alpha_{f^*}(n) = OPT$. In other words, the competitive ratio is tight when the adversary decides that the skiing stops at the end of day $n$. 

Finally, we show that for $x < n$, the only time that the competitive ratio $\alpha_{f^*}(x)$ is non-optimal is when $f_x$ cannot be increased further due to a tail constraint being violated. 

The last two invariants give a prescriptive way of computing the optimal solution. Guess the value of OPT, then start with $f_1$ so that $\alpha_{f}(1) = OPT$, then set $f_2$ such that $\alpha_{f}(2) = OPT$ and so on until one of the tail constraints gets tight. If the guess for $OPT$ is correct then the resulting $f_i$'s will form a probability distribution, as is required. If we guessed too high, then $\sum_i f_i$ will exceed 1; if we guessed too low, it will be too low. \sergei{mention the non-analytic nature of the solution?}

The prescriptive approach above hides surprising and unexpected properties of the optimal solution, which we describe in more detail below. 

\paragraph{Pure tail Constraints}
We begin with considering a single tail constraints of the form $(\gamma, 0)$, i.e. the competitive ratio is never allowed to exceed $\gamma$. We call these {\em pure} tail constraints.  A simple calculations shows that such a constraint implies that $f_i = 0$ for $i < n/(\gamma - 1)$, that is we always rent for the first $n/(\gamma - 1)$ days. Since this is the only tail constraint, the rest of the analysis relies on allocation the probability mass such that the competitiveness function on the remaining interval remains constant. The shape of the optimal solution here has a spike in probability of buying skis precisely on day $n/(\gamma - 1)$, followed by $f_i$ again being proportional to $\exp(i/n)$. 

\paragraph{Approximate Tail constraints}
While the spike in the pure tail constraint case is somewhat surprising, things get much less intuitive with approximate tail constraints. 

Here the pair of invariants we described above leads to a solution with a non-trivial shape, which we illustrate in Figure \ref{fig:xxx}. The purchase distribution, $f$,  oscillates between periods of $0$ probability of buying, together with periods of ever higher probability of buying. 

We highlight a few qualitative results about this solution. First, as $\delta$ drops to 0, the number of times the solution drops to $0$ grows without bound. Second, as $\delta$ drops to 0, the relative likelihood of one day over another non-zero day grows exponentially (this is super rough, i don't know how to phrase it --sv). Finally, the exact places where the solution oscillates are non-analytic, and are a solution involving the Lambert $W$ function. 

\subsection{Related Work}
\label{sec:related}
What should go here? Other than the one paper Bobby highlighted? 
